Understanding Human-AI Collaboration in Cybersecurity Competitions

Capture-the-Flag (CTF) competitions are increasingly becoming a testbed for evaluating AI capabilities at solving security tasks, due to the controlled environments and objective success criteria. Existing evaluations have focused on how successful AI is at solving CTF challenges in isolation from human CTF players. As AI usage increases in both academic and industrial settings, it is equally likely that human players may collaborate with AI agents to solve challenges. This possibility exposes a key knowledge gap: how do humans perceive AI CTF assistance; when assistance is provided, how do they collaborate and is it effective with respect to human performance; how do humans assisted by AI compare to the performance of fully autonomous AI agents on the same challenges. We address this gap with the first empirical study of AI assistance in a live, onsite CTF. In a study with 41 participants, we qualitatively study (i) how participants' perception, trust, and expectations shift before versus after hands-on AI use, and (ii) how participants collaborate with an instrumented AI agent. Moreover, we also (iii) benchmark four autonomous AI agents on the same fresh challenge set to compare outcomes with human teams and analyze agent trajectories. We find that, as the competition progresses, teams increasingly delegate larger subtasks to the AI, giving it more agency. Interestingly, CTF challenges solving rates are often constrained not by model's reasoning capabilities, but rather by the human players: ineffective prompting and poor context specification become the primary bottleneck. Remarkably, autonomous agents that self-direct their prompting and tool use bypass this bottleneck and outperform most human teams, coming in second overall in the competition. We conclude with implications for the future design of CTF challenges and for building effective human-in-the-loop AI systems for security.

==> 8.conc.tex <==
\section{Conclusion}

==> relwork.tex <==
\section{Related Work}

1. Agents in CTF
- focus on agent design -> ours AI assistant
- agent benchmark dataset -> fresh CTFs-> no data leakage problem
- ccs 25 -> empirical study

2. human AI interaction

- other close domains (cybersecurity tasks)

\subsection{Agents in CTF}
To support benchmarking and evaluation, several frameworks have been developed. The NYU CTF Bench \cite{shao2024nyuctfbench} introduces an open-source dataset for evaluating and comparing LLM agents in solving CTF challenges, with standardized interfaces and automated scoring mechanisms. In addition, they also have a automated pipeline which integrates advanced function calling by LLM, making it easier to call more external tools. Similarly, Cybench \cite{zhang2025cybench} provides a LLM-based agent and an evaluator, which had better task decomposition and enables structured evaluation on subtasks, achieving more granular evaluation.

Several systems have demonstrated the potential of LLM-powered agents in CTF context. For instance, CTFAgent \cite{ji2025measuring} proposed a modular framework that integrates Retrieval Augmented Generation (RAG) and interactive Environmental Augmentation, enabling effective knowledge retrieval and vulnerability exploitation. In order to improve the effectiveness of vulnerability exploitation, EnIGMA \cite{abramovich2025enigma} imported new tools and interfaces. This interactive terminal program Tools allows LM agents to utilize more tools like debuggers. Compared with NYU CTF Bench \cite{shao2024nyuctfbench}, CRAKEN \cite{shao2025craken} aimed to solve more difficult challenges by adding new security knowledge into extensible database. Other efforts such as InterCode-CTF \cite{yang2023intercode} and HackSynth \cite{muzsai2024hacksynthllmagentevaluation} both propose their agents and corresponding benches. To be specific, InterCode-CTF built on a mimic real world CTF competitions, helping agent to find vulnerabilities quicker. The dual-module architecture (planner and summarizer) in HackSynth allows agent to determine commands and process responses in each iteration, which makes it easier to modify task decomposition and direction of the solution. CTF-DOJO \cite{zhuo2025cyber, zhuo2025training} further completed a large-scale, execution-grounded training environment for LLM agents. Paired with the automated pipeline CTF-FORGE, it enables efficient and reproducible generation of executable environments. 


\subsection{Human-AI Interaction}
Human-AI interaction and collaboration have been widely studied across many domains, representing a significant focus shift to interaction \cite{fragiadakis2025evaluatinghumanaicollaborationreview}. Using for educational, financial, and healthcare goals, it have showed significant achievements \cite{buckley2021regulating, Lui2018ArtificialIA, tschandl2020human, holstein2021designinghumanaicomplementarityk12}. In a broader context, Human–AI interaction has found extensive applications across a wide range of tasks, including decision-making, strategic planning, as well as systematic verification and validation processes \cite{DBLP:journals/corr/abs-2102-05460, nargund2025understandingmodeswitchinghumanai, zhang2025jumpstarterhumanaiplanningtaskstructured}. These capabilities closely align with the core competencies emphasized in cybersecurity, thereby motivating the growing integration of AI into critical security tasks, including vulnerability identification, analysis and fix. 

In cybersecurity and related technical domains, recent work has begun to explore how human experts interact with automated tools and AI assistants. For instance, 
